Image Restoration using Feature-guidance

Image restoration is the task of recovering a clean image from a degraded version. In most cases, the degradation is spatially varying, and it requires the restoration network to both localize and restore the affected regions. In this paper, we present a new approach suitable for handling the image-specific and spatially-varying nature of degradation in images affected by practically occurring artifacts such as blur, rain-streaks. We decompose the restoration task into two stages of degradation localization and degraded region-guided restoration, unlike existing methods which directly learn a mapping between the degraded and clean images. Our premise is to use the auxiliary task of degradation mask prediction to guide the restoration process. We demonstrate that the model trained for this auxiliary task contains vital region knowledge, which can be exploited to guide the restoration network's training using attentive knowledge distillation technique. Further, we propose mask-guided convolution and global context aggregation module that focuses solely on restoring the degraded regions. The proposed approach's effectiveness is demonstrated by achieving significant improvement over strong baselines.

==> haze.tex <==
%\textbf{Network Design}
% Documents:
% We design DuRB's for this task by employing up-sampling ($up$) implemented using PixelShuffle \cite{pixelshuffle} with a convolutional layer ($ct^{l}_{1}$) in $T^{l}_{1}$ and channel-wise attention ($se$) implemented using SE-ResNet module \cite{senet} with a conv. layer ($ct^{l}_{2}$) in $T^{l}_{2}$. More details are given in the supplementary material. 

\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{1pt}
			\begin{tabular}{cccccccc}
\includegraphics[width=\widthscalesix\textwidth, height=0.08\textwidth]{haze/41_input.jpg} &
\includegraphics[bb=280 1 934 290, clip=True,width=\widthscalesix\textwidth, height=0.08\textwidth]{haze/41_dcp.jpg} &
\includegraphics[bb=280 1 934 290, clip=True,width=\widthscalesix\textwidth, height=0.08\textwidth]{haze/41_gfn.jpg} &
\includegraphics[bb=280 1 934 290, clip=True,width=\widthscalesix\textwidth, height=0.08\textwidth]{haze/41_pff.jpg} &
%\includegraphics[width=\widthscalesix\textwidth]{haze/gfn} &
\includegraphics[bb=280 1 934 290, clip=True,width=\widthscalesix\textwidth, height=0.08\textwidth]{haze/41_durn.jpg} &
\includegraphics[bb=280 1 934 290, clip=True,width=\widthscalesix\textwidth, height=0.08\textwidth]{haze/41_msppn.jpg} &
\includegraphics[width=\widthscalesix\textwidth, height=0.08\textwidth]{haze/41_outdoor_GT_x1_SR_cropped.jpg} &
\includegraphics[bb=280 1 934 290, clip=True,width=\widthscalesix\textwidth, height=0.08\textwidth]{haze/41_gt.jpg} 

				\\
				(a) Input Image&
				(b) DCP& %\hspace{\fsdttwofig} &
				(c) GFN & %\hspace{\fsdttwofig} &
				(d) PFFNet & %\hspace{\fsdttwofig} &
				%(e) GFN & % \hspace{\fsdttwofig} &
				(e) DURN & %\hspace{\fsdttwofig} &
				(f) MSPPN  &%\hspace{\fsdttwofig} & & %\hspace{\fsdttwofig} &
				(g) Ours   & %\hspace{\fsdttwofig} &
				(h) GT  
				\\
	\end{tabular}
\caption{Examples of dehazing on OHAZE Dataset.}
\label{fig:haze1}
\vspace{-0.1cm}
\end{figure*}

\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{1pt}
			\begin{tabular}{cccccccc}
\includegraphics[width=\widthscalefour\textwidth]{haze/1400_10_input.jpg} &
\includegraphics[width=\widthscalefour\textwidth, height=0.105\textwidth]{haze/5438-IndoorOutdoor_dcp.jpg} &
\includegraphics[width=\widthscalefour\textwidth,height=0.105\textwidth]{haze/5438-IndoorOutdoor_dehazenet.jpg} &
\includegraphics[width=\widthscalefour\textwidth,height=0.105\textwidth]{haze/5438-IndoorOutdoor_aod.jpg} &
\includegraphics[width=\widthscalefour\textwidth,height=0.105\textwidth]{haze/5438-IndoorOutdoor_gca.jpg} &
\includegraphics[width=\widthscalefour\textwidth]{haze/1400_10_x1_SR.jpg} &
\includegraphics[width=\widthscalefour\textwidth]{haze/1400_10_gt.jpg} 

				\\
				(a) Input Image&

				(b) DCP& %\hspace{\fsdttwofig} &
				(c) DehazeNet & %\hspace{\fsdttwofig} &
			    (d) AODNet & %\hspace{\fsdttwofig} &

				(e) GCANet & %\hspace{\fsdttwofig} &
		%\hspace{\fsdttwofig} &
				(f) Ours   & %\hspace{\fsdttwofig} &
				(g) GT  
				\\
	\end{tabular}
\caption{Qualitative comparison of dehazing results on SOTS-Indoor Dataset.}
\label{fig:haze2}
\vspace{-0.1cm}
\end{figure*}

 \begin{table*}[!t]
    \large
      \centering
      \caption{
        Quantitative evaluations on the benchmark dehazing datasets.
      %{\color{red}\textbf{Red texts}} and {\color{blue}blue texts} indicate the best and the second-best performance respectively.     $\uparrow$ and $\downarrow$ mean the better methods should achieve higher/lower score of this metric.     
      }
      \begin{adjustbox}{width=1\linewidth}
        \begin{tabu}{lcccccccccccccc}
          \tabucline[1.5pt]{}
          \multicolumn{2}{c}{\textbf{Methods}} \hspace{8pt} & DCP~\cite{He_dark}   &NLD~\cite{NLD}  & AODNet~\cite{AOD}   & MSCNN~\cite{MSCNN} & MsPPN~\cite{MsPPN} & DcGAN~\cite{DcGAN}  & GFN~\cite{GFN} & GCANet~\cite{GCANet} & PFFNet~\cite{PFFNet} &GDN~\cite{griddehazenet} & DuRN~\cite{DuRN} & MSBDN~\cite{dong2020multi} & \multicolumn{1}{c}{Ours}  \\
          \hline
          \multirow{2}[2]{*}[2pt]{SOTS~\cite{RESIDE}} & PSNR$\uparrow$  & 18.75 & 17.27 &18.80  & 17.57  &29.94   &25.37  & 24.11 & 28.13 &29.22 &31.51 &{31.92} & 33.79 &{\textbf{35.96}} \\
                & SSIM$\uparrow$  & 0.859  &  0.750   &   0.834    &  0.811     & 0.958     &  0.917     &  0.899   &  0.945   &0.954  &{0.983} & 0.980 & 0.984 & {\textbf{0.984}}
                \\ \hline
  
%%          \multirow{2}[2]{*}[2pt]{HazeRD~\cite{HazeRD}} & CIEDE2000$\downarrow$  & 14.83   & 16.40    & 13.23      & 13.80   &  15.50   & {\color{blue}12.02}    & 14.83     & 14.45     & 14.46    & 13.93    & 12.48    & {\color{red}\textbf{10.36}} \\
%%                                          & SSIM$\uparrow$       & 0.767   & 0.727    & 0.833      & 0.794   &  0.759                               & 0.826    & 0.802     & 0.819     & 0.808    & 0.833   & {\color{blue}0.840}    & {\color{red}\textbf{0.881}}
%%                 \\ \hline
  
%%          \multirow{2}[2]{*}[2pt]{I-HAZE~\cite{IHAZE}} & PSNR$\uparrow$  & 14.43 & 14.12 &  13.98& 15.22 & {\color{blue}22.50} &  16.06 &   15.84  &   14.95    &   16.01 &16.62  &21.23 & {\color{red}\textbf{23.93}} \\
%%                & SSIM$\uparrow$  & 0.752 & 0.654 &  0.732 & 0.755 & {\color{blue}0.871} &       0.733   &   0.751    &   0.719  &   0.740  &0.787 &0.842  &  {\color{red}\textbf{0.891}}
%%                 \\ \hline
  
          \multirow{2}[2]{*}[2pt]{O-HAZE~\cite{OHAZE}} & PSNR$\uparrow$  & 16.78 & 15.98 & 15.03& 17.56 & {24.24} &     19.34   &  18.16  & 16.28 &18.76  &18.92 &20.45   & 24.36 & {\textbf{25.86}} \\
                & SSIM$\uparrow$  & 0.653 &0.585  &0.539 & 0.650 & {0.721} &    0.681  &   0.671   &  0.645  &     0.669  &0.672  &0.688  & 0.749 & {\textbf{0.786}}\\
          \tabucline[1.5pt]{}
        \end{tabu}%
      \end{adjustbox}
      \label{tab:haze1}%
   \vspace{-1mm}
    \end{table*}

%The entire network (named DuRN-US) has an encoder-decoder structure similar to the DuRN-U designed for motion blur removal, as shown in Fig.~\ref{fig:DuRN_dehaze}. We stack 12 DuRB-US's in the middle of the network; the number of channels is 64 for all the layers. In the supplementary material, we demonstrate how our network estimates a transmission map inside its attention mechanisms. For this task, we employed a weighted sum of SSIM and $l_1$ loss for training the DuRN-US.
% A figure to show the dehaze_net's architecture.


 %It should be noted that the state-of-the-art method on the Dehaze Dataset, DCPDN \cite{dehaze_zhanghe}, is trained using i) hazy images, ii) ground truth images, iii) ground truth global atmosphere light , iv) ground truth transmission maps; additionally, its weights are initialized by those of DenseNet \cite{densenet}  pre-trained on the ImageNet\cite{imagenet}. The proposed DuRN-US is trained only using i) and ii).
 
We evaluate (using PSNR and SSIM) our algorithm against state-of-the-art methods based on the hand-crafted priors (DCP~\cite{He_dark} and NLD~\cite{NLD}) and CNNs (\cite{AOD,MSCNN,MsPPN,DcGAN,GFN,GCANet,PFFNet,griddehazenet,DuRN,dong2020multi}. Table \ref{tab:haze1} show quantitative results and comparisons on RESIDE-SOTS and OHAZE datasets.

As expected, the methods based on hand-crafted features~\cite{He_dark, NLD} do not perform well. The methods~\cite{AOD, MSCNN, DcGAN} that perform hand-crafted processing along with deep CNNs are less effective when the intermediate variables are not correctly estimated. On the other hand, the end-to-end networks~\cite{GCANet,PFFNet, MsPPN, DuRN, griddehazenet,dong2020multi} generate better results than the other indirect ones. The proposed method outperforms these algorithms both qualitively and quantitively. The results on the OHAZE dataset also demonstrate our superiority for dehazing large resolution images.

Figs. \ref{fig:haze1} and \ref{fig:haze2} show qualitative comparisons with existing methods for test images from OHAZE and SOTS-Indoor datasets. It is observed that our results are closer to ground-truth. %In  sub-figure (B), we show results for two real-world hazy images\footnote{The images are available from https://github.com/rwenqi/GFN-dehazing} produced by two state-of-the-art methods, GFN\cite{GFN} and DCPDN\cite{dehaze_zhanghe}, and by ours. It can be observed that our network yields the most realistic dehazed images. It is noteworthy that our DuRN-US can properly deal with strong ambient light (sunshine coming behind the girl). See the example in the left-bottom of Fig.~\ref{fig:haze_testA}.


